Rationale Dataset and Analysis for the Commit Messages of the Linux Kernel Out-of-Memory Killer

Code commit messages can contain useful information on why a developer has made a change. However, the presence and structure of rationale in real-world code commit messages is not well studied. Here, we detail the creation of a labelled dataset to analyze the code commit messages of the Linux Kernel Out-Of-Memory Killer component. We study aspects of rationale information, such as presence, temporal evolution, and structure. We find that 98.9% of commits in our dataset contain sentences with rationale information, and that experienced developers report rationale in about 60% of the sentences in their commits. We report on the challenges we faced and provide examples for our labelling.

==> tables/frequent_words.tex <==

\begin{table*}[]
\small
    \centering
     \caption{Top 10 frequent words and their count per category, without overlap}
    
    \begin{tabular}{c|c}
       \textbf{Category}  & \textbf{Top 10 frequent words and their counts} \\\hline
     
       Decision & 'add': 28,
 'use': 28,
 'remove': 28,
 'kill': 27,
 'tasks': 22,
 'set': 20,
 'cpuset': 20,
 'instead': 19,
 'introduce': 18,
 'check': 16 \\

 Rationale &   'might': 5,
 'make': 5,
 'will': 4,
 'Fixes': 4,
 'help': 4,
 'debugging': 4,
 'later': 4,
 'use': 3,
 'reduce': 3,
 'useful': 3 \\

 Supporting Facts & 'kill': 46,
 'will': 29,
 'tasks': 28,
 'node': 27,
 'killed': 26,
 'current': 26,
 'allocation': 24,
 'set': 23,
 'check': 21,
 'reaper': 20 \\
 \end{tabular}
 \label{tab:word_count}
 \vspace{-0.15in}
\end{table*}


 


\begin{comment}
%decisions 
'add': 28,
 'use': 28,
 'remove': 28,
 'kill': 27,
 'tasks': 22,
 'set': 20,
 'cpuset': 20,
 'instead': 19,
 'introduce': 18,
 'check': 16

% rationale 
{'might': 5,
 'make': 5,
 'will': 4,
 'Fixes': 4,
 'help': 4,
 'debugging': 4,
 'later': 4,
 'use': 3,
 'reduce': 3,
 'useful': 3}

% facts
 {'kill': 46,
 'will': 29,
 'tasks': 28,
 'node': 27,
 'killed': 26,
 'current': 26,
 'allocation': 24,
 'set': 23,
 'check': 21,
 'reaper': 20}
\end{comment}


==> text/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% In this section, we summarize the RQs, discuss the challenges and present the threats to validity.


%%%%%%%%%%%%%%%%%%
\subsection{Challenges}
\label{sec:challenges}
This section discusses the challenges in creating the dataset.%, as well as the insights we gained after doing the above analyses.

%% Challenges 1 : the preprocessing 
\paragraph{Challenge 1: Deficient pre-processing}
Since the data was not properly formatted, the pre-processing step was challenging and only partially successful. For instance, entries such as \textsl{``BUG: scheduling while atomic: rsyslogd/1422/0x00000002 INFO: lockdep is turned off''}\footnote{\scriptsize \url{https://api.github.com/repos/torvalds/linux/git/commits/b52723c5607f7684c2c0c075f86f86da0d7fb6d0}} were not removed. That's why  we introduced the \textit{Inapplicable} label.  In fact, we continued cleaning the data while doing the labelling. The pre-processed sentences could be also be corrected manually but that would be time consuming and error-prone. 


%% Challenges 2 : our ctaegorization 
\paragraph{Challenge 2: A high-level codebook}
The categorization of components of the rationale of commits that we have adopted from ~\cite{dhaouadi2023towards} was data-driven (e.g, the authors came to the codebook after several discussions and consolidation meetings). However, this model is preliminary and is used as a first-order classification. For example, although we labelled the sentence \textsl{``A future optimization could be to put sched\_entity and sched\_rt\_entity into a union.''}\footnote{\scriptsize \url{https://api.github.com/repos/torvalds/linux/git/commits/fa717060f1ab7eb6570f2fb49136f838fc9195a9}} as \textit{Decision}, it could also fit under a \textit{Suggestion} category. We plan to extend this codebook in the future to include other components of commit message rationale (e.g. Goal, Need, Benefit, etc.~\cite{alsafwanDevelopersNeedRationale2022}). %and to consider previous rationale representations (Section~\ref{sec:related}).


%% Challenges 3 : Difficuelt to understand messages 
\paragraph{Challenge 3: Unclear sentences.}
The main challenge faced was understanding the commit messages. In fact, it was very difficult to comprehend some commits due to  implicit or ambiguous language (especially past/future tenses). 
For instance, in the last two paragraphs in this commit\footnote{\scriptsize \url{https://api.github.com/repos/torvalds/linux/git/commits/93065ac753e4443840a057bfef4be71ec766fde9}}, 
\michalis{Hm, I don't like this. We are not submitting hypertext, so readers cannot easily access linked comment. If we want to refer to specific text from that commit, we should copy it in the paper unfortunately.}
it is difficult to distinguish between 
a) statements about the system before the patch,
b) statements about the system after the patch 
and c) future work/plans statements.
% exp: lines 130/131/132/133/134 from batch 3 
As this commit message is written by a (presumed) non-native author, it is hard to read the tense of the sentence. Finally,  most commits needed  technical understanding. %Thus, we had to look at the code and precisely understand what the commit is doing  to figure out the suitable labelling.
Although we tried our best to interpret what the sentence contains, it is still possible that we
misunderstood some of the commit messages. 
We thus relied on inclusivity in case of disagreement.
We consider as future work involving Linux developers to obtain a more reliable labelling and a finer-grained analysis. 
% that would be another project

\input{text/threats}


